STE-QUEST - Test of the Universality of Free Fall Using Cold Atom Interferometry

The theory of general relativity describes macroscopic phenomena driven by the influence of gravity while quantum mechanics brilliantly accounts for microscopic effects. Despite their tremendous individual success, a complete unification of fundamental interactions is missing and remains one of the most challenging and important quests in modern theoretical physics. The STE-QUEST satellite mission, proposed as a medium-size mission within the Cosmic Vision program of the European Space Agency (ESA), aims for testing general relativity with high precision in two experiments by performing a measurement of the gravitational redshift of the Sun and the Moon by comparing terrestrial clocks, and by performing a test of the Universality of Free Fall of matter waves in the gravitational field of Earth comparing the trajectory of two Bose-Einstein condensates of Rb85 and Rb87. The two ultracold atom clouds are monitored very precisely thanks to techniques of atom interferometry. This allows to reach down to an uncertainty in the E\"otv\"os parameter of at least 2x10E-15. In this paper, we report about the results of the phase A mission study of the atom interferometer instrument covering the description of the main payload elements, the atomic source concept, and the systematic error sources.

==> Journal_Abbreviations.tex <==
\def\aap{Astron.\ Astrophys.}
\def\aaps{Astron.\ Astrophys.\ Suppl.\ Ser.}
\def\AJ{Astron.\ J.}
\def\AN{Astron.\ Nachr.}%Astronomische Nachrichten
\def\AP{Ann.\ Phys.}
\def\APJ{Astrophys.\ J.}
\def\APJL{Astrophys.\ J.\ Lett.}


\def\BASI{Bull.\ Astron.\ Soc.\ India}%Bulletin of the Astronomical Society of India

%\def\grg{Gen.\ Relat.\ Gravit.}
\def\GRG{Gen.\ Relat.\ Gravit.} %General Relativity and Gravitation

\def\CJP{Czech.\ J.\ Phys.}
\def\CMP{Comm.\ Math.\ Phys.}
\def\CQG{Classical Quant.\ Grav.}

\def\EPL{Europhys.\ Lett.}

\def\JETP{J.\ Exp.\ Theor.\ Phys.}
\def\JETPL{J.\ Exp.\ Theor.\ Phys.\ Lett.}
\def\JGP{J.\ Geom.\ Phys.}
\def\JMP{J.\ Math.\ Phys.}
\def\JOG{J.\ Geodesy}
\def\JPA{J.\ Phys.\ A: Math.\ Gen.}%Journal of Physics A Mathematical General



\def\LMP{Lett.\ Math.\ Phys.}
\def\LRR{Living Rev.\ Relat.}

\def\MPLA{Mod.\ Phys.\ Lett.\ A}
\def\mnras{Mon.\ Not.\ R.\ Astron.\ Soc.}%{M}on.\ {N}ot.\ {R}.\ {Astron}.\ {S}oc.\
\def\MRL{Math.\ Res.\ Lett.}


\def\nat{Nature}
\def\NCB{Nuovu Cimento B}
\def\NPB{Nucl.\ Phys.\ B}

\def\pasj{Publ.\ Astron.\ Soc.\ Japan}
\def\physrep{Phys.\ Rep.}
\def\PLA{Phys.\ Lett.\ A}
\def\PNAS{PNAS } %Proceedings of the National Academy of Sciences
\def\PRD{Phys.\ Rev.\ D}
\def\pre{Phys.\ Rev.\ E}
\def\PR{Phys.\ Rev.}
\def\PRL{Phys.\\ Rev.\\ Lett.}
\def\PRSEA{Proc.\ Roy.\ Soc.\ Edinburgh A}%
\def\PRSLA{Proc.\ Roy.\ Soc.\ London A}%
\def\PTP{Prog.\ Theor.\ Phys.}
\def\PTRSL{Phil.\\ Trans.\\ R.\\ Soc.\\ Lond.\ A}




\def\QJPAM{Quart.\ J.\ Pure and Appl.\ Math.}

\def\RMP{Rev.\ Mod.\ Phys.}

\def\ZfP{Z.\ Phys.}%Zeitschrift fur Physik

